Scalable Blocking for Very Large Databases

In the field of database deduplication, the goal is to find approximately matching records within a database. Blocking is a typical stage in this process that involves cheaply finding candidate pairs of records that are potential matches for further processing. We present here Hashed Dynamic Blocking, a new approach to blocking designed to address datasets larger than those studied in most prior work. Hashed Dynamic Blocking (HDB) extends Dynamic Blocking, which leverages the insight that rare matching values and rare intersections of values are predictive of a matching relationship. We also present a novel use of Locality Sensitive Hashing (LSH) to build blocking key values for huge databases with a convenient configuration to control the trade-off between precision and recall. HDB achieves massive scale by minimizing data movement, using compact block representation, and greedily pruning ineffective candidate blocks using a Count-min Sketch approximate counting data structure. We benchmark the algorithm by focusing on real-world datasets in excess of one million rows, demonstrating that the algorithm displays linear time complexity scaling in this range. Furthermore, we execute HDB on a 530 million row industrial dataset, detecting 68 billion candidate pairs in less than three hours at a cost of $307 on a major cloud service.

==> compression-table.tex <==
%% compression and time 
%%
\newcommand{\cmpColWid}{0.8cm}
\begin{table}
	\caption{Comparing compression and elapsed time for blocking (in minutes)}
	\begin{tabular}{|p{1.4cm}|>{\centering\arraybackslash}p{\cmpColWid}|>{\centering\arraybackslash}p{\cmpColWid}|>{\centering\arraybackslash}p{\cmpColWid}|>{\centering\arraybackslash}p{\cmpColWid}|>{\centering\arraybackslash}p{\cmpColWid}|>{\centering\arraybackslash}p{\cmpColWid}|}
		\hline
		& \multicolumn{2}{c|}{Simple} & \multicolumn{2}{c|}{PMB} & \multicolumn{2}{c|}{FDB}  \\ 
		\hline
		Dataset & Comp & Time & Comp & Time & Comp & Time \\ 
		\hline
		VAR1M 	& 94.909 & 2.6	& 94.268	& 27.7		& 95.429	& 6.1 \\ 
		VAR10M 	& 96.198 & 4.8	&  			& 			& 96.387 	& 9.8 \\ 
		VAR25M 	& 96.847 & 7.8	& 			& 			& 97.369 	& 14.6 \\ 
		VAR50M 	& 97.090 & 13.9	&  			&  			& 97.683 	& 30.5 \\ 
		VAR107M & 97.290 & 23.8	&  			&  			& 97.923 	& 54.6 \\ 
		VIDEO 	& 30.084 & 3.6	& 			&  			& 34.900 	& 6.7 \\ 
		POI 	& 11.563 & 9.8	& 0.266  	& 330.9  	& 12.608 	& 13.7 \\ 
		%ABTBUY & 1.703 & 6.1 & 10.769 & 0.4 \\ 
		%GOOG & 3.073 & 6.5 & 20.876 & 0.4 \\ 
		%SCHOLAR &  & 4.7 & 10.390 & 1.0 \\ 
		%ACM &  & 3.5 & 46.945 & 0.5 \\ 
		DBPEDIA & 25.080 & 3.6	& 25.364 	& 28.0 		& 26.540 	& 20.8 \\ 
		FREEB 	& 13.519 & 6.8	& 10.414 	& 34.8 		& 15.651 	& 25.1 \\ 
		\hline
	\end{tabular}
	\label{resultsCompression}
\end{table}



==> lsh-table.tex <==
% lsh results as a table 
% 
\newcommand{\lshColWid}{0.72cm}
\begin{table}
	\caption{Impact of different LSH configurations ($b$, $w$) on compression, precision, and pairs produced}
	\begin{tabular}{|p{0.2cm}|p{1.4cm}|>{\centering\arraybackslash}p{\lshColWid}|>{\centering\arraybackslash}p{\lshColWid}|>{\centering\arraybackslash}p{\lshColWid}|>{\centering\arraybackslash}p{\lshColWid}|>{\centering\arraybackslash}p{\lshColWid}|>{\centering\arraybackslash}p{\lshColWid}|}
		\hline
		& Dataset & OFF & (1,10) & (2,9) & (3,8) & (4,7) & (5,6) \\ 
		\hline
		\multirow{4}{*}{\rotatebox[origin=c]{90}{Comp}} & VAR25M  & 94.741 & 95.909 & 96.904 & 97.369 & 97.825 & 98.323 \\ 
		& VIDEO     & 32.599 & 33.069 & 33.568 & 34.900 & 35.956 & 39.674 \\ 
		& ABTBUY   & 2.301 & 10.769 & 10.769 & 10.769 & 10.769 & 10.769 \\ 
		& SCHOLAR     & 7.891 & 8.741 & 9.386 & 10.390 & 11.207 & 12.486 \\ 
		\hline
		\multirow{4}{*}{\rotatebox[origin=c]{90}{Prec}} & VAR25M  & 40.767 & 34.930 & 30.019 & 27.393 & 21.975 & 17.151 \\ 
		& VIDEO     & 3.984 & 3.987 & 3.927 & 3.965 & 3.825 & 3.984 \\ 
		& ABTBUY   & 0.158 & 0.745 & 0.745 & 0.745 & 0.745 & 0.745 \\ 
		& SCHOLAR     & 1.339 & 1.450 & 1.530 & 1.476 & 1.468 & 1.373 \\ 
		\hline
		\multirow{4}{*}{\rotatebox[origin=c]{90}{Pairs Prod}} & VAR25M & 2.59B & 3.14B & 4.38B & 5.33B & 7.68B & 12.10B \\
		& VIDEO & 505M & 514M & 531M & 555M & 597M & 714M \\
		& ABTBUY & 31k & 33k & 33k & 33k & 33k & 33k \\
		& SCHOLAR & 546k & 583k & 605k & 727k & 811k & 1M \\
		\hline
	\end{tabular}
	\label{lshResults}
\end{table}



==> slider-table.tex <==
% recall Slider results when holding LSH slider at (3,8)
%

\newcommand{\rstColWid}{0.9cm}
\begin{table}[htbp]
	\caption{Impact of recallSlider when holding LSH constant at (3, 8)}
	\begin{tabular}{|l|p{1.4cm}|>{\centering\arraybackslash}p{\rstColWid}|>{\centering\arraybackslash}p{\rstColWid}|>{\centering\arraybackslash}p{\rstColWid}|>{\centering\arraybackslash}p{\rstColWid}|>{\centering\arraybackslash}p{\rstColWid}|}
		\hline
		 & & \multicolumn{5}{c|}{Recall Cost Slider Value} \\
		 \hline
		 & Dataset & 0.01 & 0.25 & 0.5 & 0.75 & 0.99 \\
	  	\hline
		\multirow{7}{*}{\rotatebox[origin=c]{90}{Compression}} & VAR1M & 95.044 & 95.302 & 95.429 & 95.597 & 95.723 \\ 
		& VAR10M & 96.005 & 96.246 & 96.387 & 96.519 & 96.612 \\ 
		& VAR25M & 97.079 & 97.261 & 97.369 & 97.470 & 97.549 \\ 
		& VIDEO & 30.003 & 33.192 & 35.598 & 37.286 & 38.317 \\ 
		& POI & 11.219 & 12.078 & 12.608 & 13.204 & 13.566 \\ 
		%& ABTBUY & 5.430 & 5.430 & 5.430 & 5.430 & 5.430 \\ 
		%& GOOG & 20.876 & 21.290 & 21.290 & 21.290 & 21.290 \\ 
		%& SCHOLAR & 10.390 & 10.448 & 10.536 & 10.927 & 11.367 \\ 
		%& ACM & 46.945 & 46.945 & 46.945 & 46.945 & 46.945 \\ 
		& DBPEDIA & 26.444 & 26.505 & 26.540 & 26.574 & 26.594 \\ 
		& FREEB & 14.960 & 15.388 & 15.651 & 15.989 & 16.203 \\ 
		\hline
		\multirow{7}{*}{\rotatebox[origin=c]{90}{Precision}} & VAR1M & 34.325 & 29.192 & 26.125 & 22.309 & 20.462 \\ 
		& VAR10M & 41.148 & 35.086 & 30.834 & 26.286 & 23.899 \\ 
		& VAR25M & 35.053 & 30.475 & 27.393 & 24.125 & 22.244 \\ 
		& VIDEO & 4.316 & 4.123 & 3.906 & 3.744 & 3.552 \\ 
		& POI & 1.096 & 0.865 & 0.685 & 0.500 & 0.393 \\ 
		%& ABTBUY & 0.380 & 0.380 & 0.380 & 0.380 & 0.380 \\ 
		%& GOOG & 1.536 & 1.253 & 1.253 & 1.253 & 1.253 \\ 
		%& SCHOLAR & 1.476 & 0.948 & 0.552 & 0.305 & 0.147 \\ 
		%& ACM & 53.974 & 53.974 & 53.974 & 53.974 & 53.974 \\ 
		& DBPEDIA & 0.041 & 0.029 & 0.024 & 0.018 & 0.015 \\ 
		& FREEB & 0.028 & 0.019 & 0.015 & 0.009 & 0.007 \\ 
		\hline
		\multirow{7}{*}{\rotatebox[origin=c]{90}{Pairs Produced}} & VAR1M & 76M & 123M & 164M & 226M & 284M \\ 
		& VAR10M & 656M & 1.06B & 1.42B & 2.00B & 2.57B \\ 
		& VAR25M & 2.44B & 3.96B & 5.33B & 7.47B & 9.51B \\ 
		& VIDEO & 258M & 446M & 618M & 831M & 1.01B \\ 
		& POI & 430M & 753M & 1.10B & 1.80B & 2.52B \\ 
		%& ABTBUY & 32k & 32k & 32k & 32k & 32k \\ 
		%& GOOG & 92k & 114k & 114k & 114k & 114k \\ 
		%& SCHOLAR & 727k & 1M & 1M & 3M & 8M \\ 
		%& ACM & 6k & 6k & 6k & 6k & 6k \\ 
		& DBPEDIA & 2.14B & 2.99B & 3.71B & 4.88B & 5.96B \\ 
		& FREEB & 3.74B & 5.68B & 7.57B & 12.24B & 17.29B \\ 
		\hline
	\end{tabular}
	\label{sliderResults}
\end{table}


==> token-blocking-table.tex <==

\begin{table}
	\centering
	\caption{Comparing blocking algorithms on SCHOLAR using Token Blocking and LSH-based block building strategies}
	\begin{tabular}{%
	|l|c|c|c|
	}
		\hline
		Setup & $|B|$ & $PQ$ & $PC$  \\ 
		\hline
		%
HDB TB=0.5 & $\expnum{1.04}{8}$ & $\nexpnum{3.00}{4}$ & 0.9986 \\
HDB TB=0.01 & $\expnum{2.76}{7}$ & $\nexpnum{1.07}{3}$ & 0.9963 \\
PMB TB=0.01 & $\expnum{2.83}{7}$ & $\nexpnum{1.12}{3}$ & 0.9971 \\
HDB LSH(16,3) & $\expnum{1.31}{7}$ & $\nexpnum{2.06}{3}$ & 0.9443 \\

		%
		\hline
	\end{tabular}
	\label{tbl:tokenBlockingResults}
\end{table}




